UNOPose: Unseen Object Pose Estimation with an Unposed RGB-D Reference Image

Unseen object pose estimation methods often rely on CAD models or multiple reference views, making the onboarding stage costly. To simplify reference acquisition, we aim to estimate the unseen object's pose through a single unposed RGB-D reference image. While previous works leverage reference images as pose anchors to limit the range of relative pose, our scenario presents significant challenges since the relative transformation could vary across the entire SE(3) space. Moreover, factors like occlusion, sensor noise, and extreme geometry could result in low viewpoint overlap. To address these challenges, we present a novel approach and benchmark, termed UNOPose, for unseen one-reference-based object pose estimation. Building upon a coarse-to-fine paradigm, UNOPose constructs an SE(3)-invariant reference frame to standardize object representation despite pose and size variations. To alleviate small overlap across viewpoints, we recalibrate the weight of each correspondence based on its predicted likelihood of being within the overlapping region. Evaluated on our proposed benchmark based on the BOP Challenge, UNOPose demonstrates superior performance, significantly outperforming traditional and learning-based methods in the one-reference setting and remaining competitive with CAD-model-based methods. The code and dataset are available at https://github.com/shanice-l/UNOPose.

==> tables/uno_pose_abla.tex <==
\begin{table*}[t]
    \centering
    \caption{
        {\bf Ablation study on YCB-V.}
        %
        \emph{(a):} Ablation of network architecture, GRF/LRF, correspondence loss, and segmentation.
        \emph{(b):} Ablation of initial rotation distance between query and reference objects.
    }
    %%%%%%%%%%%%%%%%%%%%%%%%%%
    \begin{subfigure}[t]{0.7\linewidth}
    \vspace{4pt}
    \tablestyle{11pt}{1.25}
	\begin{tabular}{@{}l | l | ccc | c@{}}
	% \shline
        ROW & Method & VSD & MSSD & MSPD & $\text{AR}_{\text{BOP}}$ \\
        \shline
        A0 & Coarse Refinement & 63.9 & 66.6 & 57.5 & 62.7 \\
        % A1 & Coarse-to-fine Refinement & 52.2 & 63.4 & 51.4 &  55.7 \\
        % A2 & A1: MAE ViT $\rightarrow$ Frozen DINOv2 & 56.3  & 68.6 & 55.8 & 60.2 \\
        A1 & Coarse-to-fine Refinement & 79.5& 84.2& 75.3& 79.7 \\
        A2 & A1: MAE ViT $\rightarrow$ Frozen DINOv2 &  79.8 & 85.0 & 75.5 & 80.1 \\
        \hline
        % B0 & A2+Positional Enconding & 79.8 & 85.0 & 75.5 & 80.1 \\
        B0 & A2 + GRF & 79.4 & 85.2 & 76.6 & 80.4 \\ 
        % B1 & A2 + LRF & 79.6 & 84.0 & 75.0 & 79.5 \\
        B1 & A2 + LRF & 80.6 & 84.7 & 75.8 & 80.4 \\
        B2 & A2 + GRF + LRF &  80.7 & 86.0 & 77.7 & 81.5   \\
        % B3 & B2: w/o BallGroup & 59.4 & 70.6 & 59.0 & 63.0 \\
        \hline
        C0 & B2 + Overlap Predictor & \textbf{82.6} & \textbf{87.4} & \textbf{79.4} & \textbf{83.1} \\
        C1 & B2 + Soft Correspondence~\cite{yu2021cofinet} & 77.1 & 81.7 & 72.7 & 77.2 \\
        \hline 
        F0 & C0: Seg. $\rightarrow$ CNOS~\cite{nguyen2023cnos} & 77.4 & 80.9 & 73.6 &  77.3 \\
        F1 & C0: Seg. $\rightarrow$ SAM-6D~\cite{lin2023sam6d} & 78.3 & 82.1 & 74.3 &  78.2 \\
        F2 & C0: Seg. $\rightarrow$ MRCNN~\cite{maskrcnn,labbe2020cosypose} & 81.2 & 85.7 & 77.9 & 81.6 \\
    % \shline
    \end{tabular}
    \vspace{4mm}
    \caption{\label{tab:pose_abla}}
    \end{subfigure}~~~%\hfill
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \begin{subfigure}[t]{0.29\linewidth}
        \vspace{0pt}
        \includegraphics[width=0.8\linewidth]{tables/ref_rot_err_v2_bar_times.pdf}% \vspace{-2mm}
        \caption{\label{fig:pose_abla}}
    \end{subfigure}\hfill
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \vspace{-5mm}
% \captionlistentry[figure]{figure and table}
% \captionsetup{labelformat=andtable}
\end{table*}


